Angular Gap: Reducing the Uncertainty of Image Difficulty through Model Calibration

Curriculum learning needs example difficulty to proceed from easy to hard. However, the credibility of image difficulty is rarely investigated, which can seriously affect the effectiveness of curricula. In this work, we propose Angular Gap, a measure of difficulty based on the difference in angular distance between feature embeddings and class-weight embeddings built by hyperspherical learning. To ascertain difficulty estimation, we introduce class-wise model calibration, as a post-training technique, to the learnt hyperbolic space. This bridges the gap between probabilistic model calibration and angular distance estimation of hyperspherical learning. We show the superiority of our calibrated Angular Gap over recent difficulty metrics on CIFAR10-H and ImageNetV2. We further propose Angular Gap based curriculum learning for unsupervised domain adaptation that can translate from learning easy samples to mining hard samples. We combine this curriculum with a state-of-the-art self-training method, Cycle Self Training (CST). The proposed Curricular CST learns robust representations and outperforms recent baselines on Office31 and VisDA 2017.

==> agExperiment.tex <==


\section{Experiments}
We evaluate the correlation between Angular Gap and human selection frequency on CIFAR10-H\cite{Battleday2020CapturingHC} and ImageNetV2\cite{recht2019imagenet}. We further test the proposed difficulty estimation on a particularly popular curriculum learning paradigm introduced by Bengio\cite{Bengio2009CurriculumL}.
Angular Gap consistently outperforms baselines in our correlation study and downstream curricular image classification.\\
\subsection{Datasets}
CIFAR10\cite{krizhevsky2009learning} and ISLRVC 2012 \cite{deng2009imagenet} are standard training sets for image classification test. CIFAR10 contains 50,000 tiny-images for 10 classes, and ISLRVC2012 contains 1.28 million large-scale images for 1000 classes. For evaluation, CIFAR10-H\cite{Battleday2020CapturingHC} and ImageNetV2\cite{recht2019imagenet} are two recently popular behavioral datasets that report human selection frequency. Human selection frequency (HSF), is the faction of people that attend and correctly classify the current image. CIFAR10-H has 10K natural images from CIFAR10 test set with 511,400 decisions given by 2570 annotators. ImageNetV2 has 10,000 large-scale for 1000 classes. Each image has been labelled by at least 10 MTurk workers, or possibly more.
\subsection{Implementation Details}
For data prepossessing, we follow PyTorch examples\cite{NEURIPS2019_9015} to generate random image crops. For backbone feature extractors, we adopt widely used CNN architectures including AlexNet, VGG16, ResNet18, ResNet50 and ResNet101. Angular discrimination is emphasized by normalized softmax loss with a rescaling factor $s$ of 30.\\ We train the models from scratch on CIFAR datasets for 100 epochs with a batch size of 128. We set the initial learning rate as 0.1 and apply a cosine learning rate annealing strategy. On ISLRVC2012, we finetune pretrained backbones with the additive cosine margin loss to capture discriminative angular features. We set SGD momentum to 0.9, weight decay to $5e-4$, and batch size as 256. The learning rate starts from 0.1 and is divided by 10 at 30, 60 and 90 epochs, similar with\cite{he2016deep}. \\
For class-wise model calibration, we follow recent papers \cite{guo2017calibration}\cite{nixon2019measuring} and set the initial weights of vector scaling as an identity matrix. We randomly select 10\% of training samples of CIFAR10 for post-training calibration. For ISLRVC 2012, we use the validation datasets provided by the organizers. We optimize loss functions \ref{eq:globalloss} and \ref{eq:classloss} with LBFGS for 10 epochs with a learning rate of 0.01. After convergence, users can visualize class clusters, view input images and examine Angualr Gap difficulties from hypersphere.\\
We investigate image difficulties on standard curriculuml learning for further insights. With a fixed easy-to-hard order, we use the paced learning (PL) setup to fairly compare Angular Gap with other difficulty measurements. That is, we strictly follow the easy-to-hard principle \cite{Bengio2009CurriculumL, hacohen2019power} as a fixed order during data loading. We add a fraction of new hard examples at the tail of our training data every epoch. Following \cite{wu2020curricula}, we use ResNet18, linear pacing functions and grid search curriculum parameters. For each search cell, we run the same configuration with three random seeds fixed as $\{7777, 8888, 9999\}$. To ensure consistency, we employ the standard image augmentation and SGD optimization used in\cite{NEURIPS2019_9015} for CIFAR10-H. To amplify the effects of different difficulties, we apply cosine learning rate annealing. All experiments in this part use this configuration.
\begin{figure}[htbp]
\centering
\subfigure[]{
\includegraphics[width=3.7cm]{./uncertainty/ag/resnet18cifar10_AG_nsl.png}
}
\quad
\subfigure[]{
\includegraphics[width=3.7cm]{./uncertainty/ag/resnet18cifar10diagonal_scalingag_AG_nsl.png}
}
\quad
\subfigure[]{
\includegraphics[width=3.7cm]{./uncertainty/avh/resnet18cifar10_avh_nsl.png}
}
\quad
\subfigure[]{
\includegraphics[width=3.7cm]{./uncertainty/avh/resnet18cifar10diagonal_scalingag_avh_nsl.png}
}
\quad
\subfigure[]{
\includegraphics[width=3.7cm]{./uncertainty/ece/resnet18cifar10ag_calibrate_ece_nsl.png}
}
\quad
\subfigure[]{
\includegraphics[width=3.7cm]{./uncertainty/ece/resnet18cifar10diagonal_scalingag_calibrate_ece.png}
}
\caption{Comparison between uncalibrated and image difficulty calibrated at class-level on CIFAR10-H. Shadows in the plots denote the corresponding standard deviations. The first row compares Angular Gap and Angular Gap calibrated at class-level in (a) and (b) correspondingly. The second row compares AVH (c) and AVH calibrated by vector scaling (d). (e) and (f) show ECE before and after the proposed classwise calibration. Classwise model calibration reduces uncertainty in image difficulty estimation.}
\label{calibrate_uncertainty}
\end{figure}
\input{imagenetv2}
\input{standard_cl}



==> cifar10h.tex <==
\begin{table}[!htb]
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lcccc@{}}
\toprule
        & \multicolumn{2}{c}{Spearman's rank}& \multicolumn{2}{c}{Kendall's Tau} \\
\cmidrule{2-5}
&  $\rho$ & p-value & $\tau$ & p-value \\
\midrule
Maximum Confidence & 0.272$\pm$0.056 &$<$0.001       & 0.145$\pm0.038$ &$<$0.001 \\
Classification margin & 0.279$\pm$0.056&$<$0.001   & 0.142$\pm$0.040 &$<$0.001 \\
Classification margin (TS\footnote{"TS" refers to temperature scaling.}) & 0.293$\pm$0.044&$<$0.001   & 0.242$\pm$0.038 &$<$0.001 \\
C-Score\cite{Jiang2020CharacterizingSR} & 0.366$\pm0.009$         &$<$0.001  & 0.243$\pm0.006$ &$<$0.001   \\
Forgetting Events\cite{Toneva2019AnES} & 0.260$\pm0.019$  &0.048 & 0.187$\pm0.011$ &0.054 \\
Prediction Depth\cite{baldock2021deep} &0.290$\pm0.009$&$<$0.001 & 0.183$\pm0.08$&$<$0.001   \\
AVH (Global)\cite{chen2020angular} & 0.376$\pm$0.010&$<$0.001      & 0.263$\pm$0.007 &$<$0.001\\
\midrule
Angular Gap (Global) & 0.381$\pm$0.010&$<$0.001 &0.268$\pm$0.007&$<$0.001\\
Angular Gap (Class) & \underline{0.384}$\pm$0.008&$<$0.001 &\underline{0.272}$\pm$0.006&$<$0.001\\
\bottomrule
\end{tabular}
} %< \resizebox
\caption{Correlation analysis between difficulty and HSF on CIFAR10-H.}
\label{tab:cifar10h}
\end{table}

==> imagenetv2.tex <==
\begin{table}[!htp]
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lcccc@{}}
\toprule
        & \multicolumn{2}{c}{Spearman's rank}& \multicolumn{2}{c}{Kendall's Tau} \\
\cmidrule{2-5}
&  $\rho$ & p-value & $\tau$ & p-value \\
\midrule
Maximum Confidence & 0.273 &$<$0.001  & 0.201 &$<$0.001 \\
Classification margin & 0.275&$<$0.001   & 0.204 &$<$0.001 \\
Forgetting Events\cite{Toneva2019AnES} & 0.260  &0.048 & 0.187 &0.054 \\
Prediction Depth\cite{baldock2021deep}& 0.308  &$<$0.001 & 0.192 &$<$0.001\\
Classification margin (TS) & 0.293&$<$0.001   & 0.242 &$<$0.001 \\
AVH (Global)\cite{chen2020angular} & 0.377&$<$0.001      & 0.257 &$<$0.001\\
\midrule
Angular Gap (Global) & 0.379&$<$0.001 &0.269&$<$0.001\\
Angular Gap (Class) & \underline{0.382}&$<$0.001 &\underline{0.271}&$<$0.001\\
\bottomrule
\end{tabular}
} %< \resizebox
\caption{
% 
Correlation analysis between difficulty and HSF on ImageNetV2.
% 
} % \caption
\label{tab:imagenetv2}
\end{table}

==> standard_cl.tex <==
\begin{table}[]
    \centering
    \caption{Performance of difficulty trained with cross-entropy and normalized softmax loss (NSL) on CIFAR10-H}
    \begin{tabular}{ccc}
    \toprule
         Methods& Cross-Entropy&NSL \\
         \midrule
         Forgetting Events&20.2$\pm$0.9&23.2$\pm$1.0\\
         Prediction Depth&19.5$\pm$0.5&22.0$\pm$0.7\\
         C-score&\textbf{19.4$\pm$0.2}&-\\
         MC-Dropout&22.9$\pm$1.8&-\\
         Classification Margin&22.9$\pm$0.4&19.5$\pm$0.4\\
         AVH&23.4$\pm$0.6&19.8$\pm$0.4\\
         Angular Gap (Ours)&22.8$\pm$0.5&\textbf{19.4$\pm$0.4}\\
    \bottomrule
    \end{tabular}
    
    \label{tab:std_cl}
\end{table}
